Efficient and Compact Spreadsheet Formula Graphs

Spreadsheets are one of the most popular data analysis tools, wherein users can express computation as formulae alongside data. The ensuing dependencies are tracked as formula graphs. Efficiently querying and maintaining these formula graphs is critical for interactivity across multiple settings. Unfortunately, formula graphs are often large and complex such that querying and maintaining them is time-consuming, reducing interactivity. We propose TACO, a framework for efficiently compressing formula graphs, thereby reducing the time for querying and maintenance. The efficiency of TACO stems from a key spreadsheet property: tabular locality, which means that cells close to each other are likely to have similar formula structures. We leverage four such tabular locality-based patterns and develop algorithms for compressing formula graphs using these patterns, directly querying the compressed graph without decompression, and incrementally maintaining the graph during updates. We integrate TACO into an open-source spreadsheet system and show that TACO can significantly reduce formula graph sizes. For querying formula graphs, the speedups of TACO over a baseline implemented in our framework and a commercial spreadsheet system are up to 34,972x and 632x, respectively.

==> backup-sec-experiment.tex <==
\begin{figure*}[!t]
  \begin{tabular}{ccc}
      \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=0.82\linewidth]{fig/run-total-slow.pdf}
        \caption{RunTotalSlow spreadsheet \\ \hfill}
        \label{fig:run_total_slow}
      \end{minipage} 
      \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=0.92\linewidth]{fig/rate.pdf}
        \caption{Rate spreadsheet \\ \hfill}
        \label{fig:rate}
      \end{minipage}
      \begin{minipage}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/modification.pdf}
        \caption{Modify parts of RunTotalSlow to RunTotalFast in Figure~\ref{fig:locality_example}}
        \label{fig:modification}
      \end{minipage} 
  \end{tabular}
  \vspace{-7mm}
\end{figure*}

\section{Experiments}
\label{sec:exp}

Our experiments address the following research questions:
\begin{tightitemize}
    \item How much does \sys reduce the time of finding dependents and returning control to users compared to the baselines of adopting an uncompressed formula graph and a compressed formula graph for spreadsheet from prior work~\cite{Antifreeze}? (Section~\ref{sec:exp_return_control})
    
    \item How much does \sys reduce the time of building a formula graph compared to the baselines?
    (Section~\ref{sec:exp_build_graph})
    
    \item How much faster does \sys process an update on the formula graph compared to the baselines?
    (Section~\ref{sec:exp_modify_graph})
    
    \item How much does \sys reduce the formula graph sizes for a real-world spreadsheet dataset?
    (Section~\ref{sec:exp_graph_size})
    
\end{tightitemize}

\subsection{Implementation}
\label{sec:implementation}

\sys is implemented in \ds~\cite{demo1, datamodels, dataspread-demo2}, 
an open-source spreadsheet system. 
\ds combines a spreadsheet front-end with a database back-end,
supporting data beyond main memory~\cite{hutchins1985direct}.
It provides a web interface to users, 
utilizes a web server to process the requests from the web interface, 
and adopts PostgreSQL as its back-end storage manager. 
\ds uses ZK Spreadsheet~\cite{zk_spreadsheet} as its formula engine. 

As introduced in Section~\ref{sec:background}, 
\ds uses an asynchronous execution model to process an update. 
It returns control to users after it has identified all of the 
dependents of an update and marked them dirty. 
\ds maintains a formula graph to find the dependents of an update. 
\sys is implemented as a drop-in replacement for \ds's formula graph. 
It builds the compressed formula graph 
when a spreadsheet is loaded into the system and the dependencies are parsed. 
To quickly find vertices (i.e., represented as ranges) 
that overlap with a given update in a formula graph, 
we further build a R-Tree~\cite{r-tree}. 
When formula cells are updated, \ds internally 
interprets the updates as a sequence of deletes and updates of the dependencies, 
and modifies the compressed formula graph and R-Tree correspondingly. 
The compressed formula graph is stored in the database as a relation, 
where each tuple stores a compressed edge, 
which includes the attributes of 
the spreadsheet name, precedent, dependent, pattern type, 
and metadata information of this edge. 
The R-Tree indices are on the precedent and dependent attributes. 
The compressed formula graph and R-Tree can also be cached in the web server. 
In this case, the cached formula graph is implemented using an adjacency list. 

\begin{figure*}[!t]
  \begin{tabular}{cc}
      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/exp_plots/rq1/RunningTotalFast_DB_small.pdf}
        \vspace{-3mm}
        \subcaption{RunningTotalFast (small dataset)}
        \label{fig:rq1_db_small_fast}
      \end{minipage} 
      
      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/exp_plots/rq1/RunningTotalSlow_DB_small.pdf}
        \vspace{-3mm}
        \subcaption{RunningTotalSlow (small dataset)}
        \label{fig:rq1_db_small_slow}
      \end{minipage} 

      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/exp_plots/rq1/Rate_DB_small.pdf}
        \vspace{-3mm}
        \subcaption{Rate (small dataset)}
        \label{fig:rq1_db_small_rate}
      \end{minipage} \\

      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/exp_plots/rq1/RunningTotalFast_DB_big.pdf}
        \vspace{-3mm}
        \subcaption{RunningTotalFast (big dataset)}
        \label{fig:rq1_db_big_fast}
      \end{minipage} 

      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/exp_plots/rq1/RunningTotalSlow_DB_big.pdf}
        \vspace{-3mm}
        \subcaption{RunningTotalSlow (big dataset)}
        \label{fig:rq1_db_big_slow}
      \end{minipage}

      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{fig/exp_plots/rq1/Rate_DB_big.pdf}
        \vspace{-3mm}
        \subcaption{Rate (big dataset)}
        \label{fig:rq1_db_big_rate}
      \end{minipage}
  \end{tabular}
  \vspace{-3mm}
  \caption{Time of returning control to users when formula graphs are stored in the database}
  \label{fig:rq1_db}
  \vspace{-5mm}
\end{figure*}


\begin{figure}[!t]
  \begin{tabular}{cc}
      \begin{minipage}[b]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq1/mem_small.pdf}
        \vspace{-5mm}
        \subcaption{10K Rows}
        \label{fig:rq1_mem_small}
      \end{minipage} 

      \begin{minipage}[b]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq1/mem_big.pdf}
        \vspace{-5mm}
        \subcaption{500K Rows}
        \label{fig:rq1_mem_big}
      \end{minipage}
  \end{tabular}
  \vspace{-3mm}
  \caption{Time of returning control to users when formula graphs are cached in the web server}
  \label{fig:rq1_mem}
  \vspace{-7mm}
\end{figure}

\subsection{Benchmark, Baselines, and Configurations}
\label{sec:benchmark_baselines}

\stitle{Benchmark}
Our tests are based on Enron spreadsheet dataset~\cite{Enron} 
For the experiments evaluating the performance of 
finding dependents and returning control to users, 
and the experiments testing the time for building the formula graph, 
we use three spreadsheet benchmarks that
represent the common usage patterns 
based on a survey of spreadsheet users~\cite{Antifreeze} and Enron dataset~\cite{Enron},
drawn from prior work. 

The first spreadsheet, \textbf{RunTotalFast}, is shown 
in Figure~\ref{fig:locality_example} from the introduction. 
Each formula cell in column \code{B} references a cell to its left, 
which can be represented as the \rr pattern in \sys. 
In addition, each formula cell starting from \code{B2} references 
its cell above. This pattern is captured as \rrChain in \sys. 
Therefore, this spreadsheet can be compressed into two edges, 
irrespective of the number of rows. 
The second spreadsheet, \textbf{RunTotalSlow}, is shown in Figure~\ref{fig:run_total_slow}. 
In RunTotalSlow, each formula cell \code{Bi} 
takes the summation of the values from \code{A1} to \code{Ai}. 
This set of formulae have the same semantics as RunTotalFast, but use a different implementation. 
It follows the pattern \fr since each formula cell in column \code{B} 
references a range that starts at \code{A1} (i.e., fixed start) 
and ends at the cell to its left (i.e., relative end), 
and therefore can be compressed into one edge in \sys.
The third spreadsheet as shown in Figure~\ref{fig:rate} is named \textbf{Rate}. 
In Rate, each formula cell \code{Ci}  
multiplies the value of \code{Bi} by a fixed value in \code{A1} (i.e., the rate). 
The dependencies between \code{Bi} and \code{Ci} 
are compressed using the \rr pattern in \sys, 
and the fixed references to \code{A1} are represented as \ff. 

For the experiments evaluating the time of maintaining the formula graph 
with respect to updates, we initialize a spreadsheet as RunTotalSlow, 
change a subset of formulae $\code{Bi}=\code{SUM(A1:Ai)}$ starting from \code{B2} 
to the formulae $\code{Bi}=\code{Ai+B(i-1)}$ as in RunTotalFast, 
and test the time of updating the formula graph with respect to the change. 
Figure~\ref{fig:modification} shows an example of such modification. 
Finally, we run \sys's compression algorithm on the full Enron dataset, 
which includes more than 17k spreadsheets, and report how much 
\sys can reduce formula graph sizes for real-world spreadsheets. 

\stitle{Baselines}
We compare \sys with two baselines: an uncompressed formula graph 
and a compressed formula graph for spreadsheets from a recent paper~\cite{Antifreeze}. 
Both baselines were already implemented in \ds, ensuring a fair comparison. 
The uncompressed formula graph (denoted \textbf{\nocomp}) 
is stored in the database as a relation, 
where each tuple stores an edge of this graph, 
which includes the spreadsheet name, precedent, dependent of this edge. 
We also build R-Tree indices on the precedent and dependent columns. 
We use a recursive self-join between the precedent and dependent column 
to find dependents.  
We also test the case where \nocomp's formula graph and R-Tree indices 
are fully cached in the web server. 
In this case, the formula graph is implemented using an adjacency list 
and we use a modified breadth-first-search (BFS) algorithm to 
find the dependents of an update without involving any database operations. 
The difference from a regular BFS algorithm is that 
when we find the direct dependents of an update, 
we need to find the direct dependents of all of the vertices 
that overlap with the update, which is done by the R-Tree index. 

The other baseline (denoted \textbf{\anti}) is from a recent paper~\cite{Antifreeze} 
that uses asynchronous execution and a graph of compressed dependencies
to quickly return control to users when processing an update. 
\anti builds the compressed graph using the following steps. 
First, \anti builds an uncompressed formula graph 
for the dependencies. 
Then, for each cell, \anti finds its dependents and compresses them by 
finding a set of bounding ranges that contain these dependents. 
For example, assume \code{A1}'s dependents 
are \code{B1}, \code{C2}, and \code{D5}. 
If \anti is configured to find two bounding ranges, 
it will merge \code{B1} and \code{C2} into the range \code{(B1:C2)} and the 
dependents of \code{A1} are compressed as \code{(B1:C2)} and \code{D5}.
Since the bounding ranges contain false positive dependents, 
\anti proposes a greedy algorithm to find the bounding ranges 
that reduce false positive cells. 
Finally, each cell along with their compressed dependents 
are stored as a look-up table, 
which is referred to as the \textit{compressed formula graph} in \anti.

The benefit of this approach is that finding dependents only requires 
a single look-up operation, regardless of whether the compressed formula graph 
is cached in the web server or stored in the database. 
However, the cost of building it is high. 
Maintaining the compressed formula graph is also costly because 
\anti will first modify the original uncompressed formula graph 
and then rebuild the compressed graph from the uncompressed counterpart. 
%In addition, the dependents of \anti can return false positive dependents, 
%which falsely marks clean cells as dirty and reduces the interactivity of spreadsheets; 
%\sys does not return false positive dependents. 
In our experiments, we configure the number of bounding ranges to 20, as suggested 
in the original paper~\cite{Antifreeze}.

\stitle{Configurations}
All experiments are run on a machine that has 12 GB of main memory 
and one Intel i7-10750H Processor with 6 physical cores, and use Ubuntu 20.04 as the OS. 
We use a single thread for all experiments, run each test three times, 
and report the average number. 
We configure \ds to use asynchronous execution model 
and adopt PostgreSQL 10.5 as its back-end database. 
We use the default configuration of PostgreSQL.

\begin{figure*}[!t]
  \begin{tabular}{cc}
      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq2/RunningTotalFast_DB_small.pdf}
        \subcaption{RunningTotalFast}
        \label{fig:rq2_db_small_fast}
      \end{minipage} 

      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq2/RunningTotalSlow_DB_small.pdf}
        \subcaption{RunningTotalSlow}
        \label{fig:rq2_db_small_slow}
      \end{minipage}

      \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq2/Rate_DB_small.pdf}
        \subcaption{Rate}
        \label{fig:rq2_db_small_rate}
      \end{minipage}
      
  \end{tabular}
  \vspace{-3mm}
  \caption{Time of building the formula graph}
  \label{fig:rq2_db_small}
  \vspace{-5mm}
\end{figure*}

\begin{figure}[!t]
  \begin{tabular}{cc}
      \begin{minipage}[b]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq3/RefreshCache_DB_small.pdf}
        \subcaption{Small dataset}
        \label{fig:rq3_db_small}
      \end{minipage} 

      \begin{minipage}[b]{0.47\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/exp_plots/rq3/RefreshCache_DB_big.pdf}
        \subcaption{Big dataset}
        \label{fig:rq3_db_big}
      \end{minipage} 
  \end{tabular}
  \vspace{-3mm}
  \caption{Time of finishing the modification}
  \label{fig:rq3_db}
  \vspace{-7mm}
\end{figure}

\subsection{Returning Control to Users}
\label{sec:exp_return_control}

We now test the time taken for returning control to users given a spreadsheet update, 
which is dominated by the time of finding dependents in a formula graph. 
We generate the three spreadsheets in Figure~\ref{fig:locality_example} 
and Figure~\ref{fig:run_total_slow}-\ref{fig:rate} with varied number of rows. 
We report the time of returning control to users 
when processing the update on the cell \code{A1} 
because this cell has the most dependents in each spreadsheet. 
For \sys and the two baseline approaches, we test two scenarios: 
the formula graph and auxiliary data structures (e.g., an R-Tree) 
are stored in the database or cached in the web server. 

Figure~\ref{fig:rq1_db} shows the experimental results 
when we store formula graphs in the database. 
In Figure~\ref{fig:rq1_db_small_fast}-\ref{fig:rq1_db_small_rate}, we vary the 
number of rows for each spreadsheet from 5k to 25k with an interval of 5k. 
We see that \sys uses much less time of returning control to users than \nocomp. 
In addition, the execution time for \sys stays the same 
while \nocomp's execution time becomes higher as we increase the number of rows. 
This is because \sys can compress the dependencies into at most two edges 
for the three spreadsheets, 
irrespective of the number of rows of the spreadsheets. 
Finding dependents in \sys only requires two look-up operations in the database. 
\nocomp, on the other hand, does not compress the dependencies 
and its formula graph sizes are linearly growing with respect to the number of rows.
It is time-consuming for \nocomp to find the dependents of \code{A1} 
via recursive self-join. 
\anti has similar performance to \sys because it only requires one look-up operation. 
However, building the compressed formula graph for \anti is so time-consuming 
that many tests cannot finish within 30 minutes. 
Specifically, \anti did not finish after 20k rows for Rate and after 15k rows for 
the other two spreadsheets. 
In Section~\ref{sec:exp_build_graph}, we will test the time for building formula graphs. 

To highlight \sys's benefit of reducing the time of returning control to users, 
we test a set of bigger spreadsheets. Specifically, we vary the number of rows 
from 100k to 500k with an interval of 100k;
the results are shown in Figure~\ref{fig:rq1_db_big_fast}-\ref{fig:rq1_db_big_rate}. 
Note that \anti is not included in these figures because it cannot finish within 30 minutes. 
We see that the time of returning control to users for \nocomp is as high as 32s  
and \sys only takes at most 3.3ms. 

Next, we test the scenario where the formula graphs and auxiliary data structures 
are cached in the web server. We test 10k and 500k rows for the three spreadsheets;
the results are shown in Figure~\ref{fig:rq1_mem}. 
Note that in Figure~\ref{fig:rq1_mem}, 
``Slow'' and ``Fast'' represent the RunTotalSlow and RunTotalFast 
spreadsheets, respectively.
The observation from these figures is consistent with the one in Figure~\ref{fig:rq1_db}. 
\nocomp has much higher execution time than \sys and \anti even though 
it uses an in-memory BFS search instead of a recursive self-join. 
Specifically, the time of returning control to users for \nocomp 
is up to 10s while \sys only takes up to 3.6ms. 

\subsection{Building a Formula Graph}
\label{sec:exp_build_graph}

In this subsection, we evaluate the time taken for building a formula graph 
given a set of dependencies and then storing the formula graph 
in the database for all three approaches. 
Recall that \anti needs to initialize an uncompressed formula graph 
using the input dependencies and then build the compressed formula graph 
based on the uncompressed one. 
To show the best performance of \anti, we assume we have enough memory 
to cache its two formula graphs. 
For \sys, we maintain a small cache that can store up to 100 compressed edges. 
This small cache is used to accelerate finding the candidate edges 
that a new dependency can compressed into. 
For \nocomp, this a cache does not improve its performance 
since it directly writes the dependencies into the database. 
We vary the number of rows from 5k to 25k with an interval of 5k; 
the results are shown in Figure~\ref{fig:rq2_db_small}. 

We see that building a formula graph in \sys is much faster 
than both \nocomp and \anti. 
This is because compared to \nocomp, which writes all of the edges into the database, 
\sys compresses the dependencies into at most 2 edges for all three spreadsheets 
and only needs to write the compressed edges into the database. 
For \anti, its performance is dominated 
by the costly process of building the compressed formula graph. 
\nocomp and \anti take up to 65s and 26mins to build formula graphs, respectively, 
while \sys takes at most 80ms. 

\subsection{Modifying a Formula Graph}
\label{sec:exp_modify_graph}

Our next experiment is to evaluate the time taken for 
modifying a formula graph for all three approaches. 
Specifically, we test the case shown in Figure~\ref{fig:modification} 
where we initialize a RunTotalSlow spreadsheet and 
modify the first $N$ rows in column $B$ 
into the formula cells in RunTotalFast, 
which can be done by a program in practice. 
\ds interprets this modification as a list of deletes and inserts 
of the modified formula cells 
and we report the time of processing them. 
The setups for \sys, \anti, and \nocomp are the same as the previous subsection: 
we assume \anti can cache both formula graphs, 
\sys maintains a small cache that can store up to 100 edges, 
and \nocomp does not maintain a cache and directly deletes/inserts dependencies 
from/to the database. 

Our first experiment initializes 10k rows 
and varies the number of modifying rows from 2k to 10k with an interval of 2k. 
The results in Figure~\ref{fig:rq3_db_small} show that 
\sys has much lower execution time compared to both \anti and \nocomp. 
This is because \sys can modify the compressed edges without having to decompress it 
such that \sys still has a small compressed graph when processing the modification. 
When \sys finishes the modification, it then flushes the small formula graph into the database. 
\nocomp, on the other hand, has a large formula graph stored in the database. 
Modifying this large formula graph requires many database operations and is time-consuming. 
\anti will update the original uncompressed formula graph by applying the deletes and inserts, 
and rebuild the compressed counterpart, which is a costly operation. 
%as shown in Section~\ref{sec:exp_build_graph}. 
Specifically, \sys takes at most 1.1s to finish the modification, 
but \anti and \nocomp take up to 15min and 44s, respectively.

We additionally perform another experiment with 500k rows, 
varying the number of modifying rows from 100k to 500k with an interval of 100k; 
the results are shown in Figure~\ref{fig:rq3_db_big}. 
We see that \nocomp cannot finish the tests that modify 200k rows or more within 30 minutes, 
but \sys can finish all tests and take up to 41s to finish the most costly modification (i.e., modify 500k rows). 

\subsection{Compressed Formula Graph Sizes}
\label{sec:exp_graph_size}

\begin{table}[!t]
    \fontsize{8.25}{10}\selectfont
    \begin{tabular}{lllll}
    \toprule
    {} &          max & 75th per. & median &     mean \\
    \midrule
    Comp. Ratio (Edges)    &      9,508.0 &      15.0 &    6.4 &     44.0 \\
    Comp. Ratio (Vertices) &     14,262.0 &      16.0 &    7.4 &     60.4 \\
    Edges reduced          &    700,155.0 &   1,169.5 &  230.0 &  2,884.0 \\
    Vertices reduced       &  1,051,143.0 &   2,039.0 &  415.0 &  5,039.3 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of formula graph sizes between \sys and \nocomp}
    \label{tbl:exp_graph_size}
    \vspace{-7mm}
\end{table}


\begin{table}[!t]
    \fontsize{8.25}{10}\selectfont
    \begin{tabular}{lllll}
    \toprule
    {} &        max & 75th per. & median &     mean \\
    \midrule
    RR        &  525,026.0 &     850.8 &  171.0 &  2,214.9 \\
    RF        &      389.0 &       0.0 &    0.0 &      0.1 \\
    FR        &    2,997.0 &       0.0 &    0.0 &      2.8 \\
    FF        &  207,235.0 &      13.0 &    0.0 &    509.3 \\
    RR-Chain  &   24,594.0 &       5.0 &    0.0 &     77.4 \\
    RR-GapOne &   19,419.0 &      16.0 &    1.0 &     79.5 \\
    \bottomrule
    \end{tabular}
    \caption{Edges reduced for each \sys's compression pattern}
    \label{tbl:exp_pattern_size}
    \vspace{-8mm}
\end{table}

We now test the effectiveness of \sys reducing the formula graph sizes 
for Enron dataset, which includes 17k spreadsheets. 
We analyze 7.3k out of 17k spreadsheets 
by skipping the spreadsheets that cause exceptions (e.g., requiring password), 
include cross-sheet reference (which currently is not supported by \ds), 
and are too small (i.e., including less than 10 formula cells). 
For each spreadsheet with an original graph $G^\prime (E^\prime, V^\prime)$ 
and compressed graph $G(E, V)$, 
we compute four metrics: 
the compression ratios with respect to edges and vertices 
(i.e., $\frac{|E^\prime|}{|E|}$ and $\frac{|V^\prime|}{|V|}$), 
and the number of reduced edges or vertices (i.e., $|E^\prime| - |E|$ and $|V^\prime| - |V|$).
We report the maximum value, the 75th percentile (denoted 75th per. for short), 
the median, and the mean value for each of the four metrics 
across the 7.3k spreadsheets; 
Table~\ref{tbl:exp_graph_size} shows the experimental results. 

We see that \sys can significantly reduce the graph sizes. 
The compression ratios with respect to edges and vertices 
are up to more than 9k and 14k, respectively, 
and both average compression ratios are more than 44. 
\sys's compressed formula graph reduces up to more than 700k 
edges and more than 1M vertices compared to the uncompressed formula graph. 

We further report the number of edges reduced by each pattern. 
For each spreadsheet, we find the compressed edges $E_p$ corresponding to a pattern $p$ 
and the uncompressed edges $E^\prime_p$ from the original graph that are compressed into $E_p$. 
Then, the number of edges reduced by $p$ is $|E^\prime_p|-|E_p|$.  
We report the maximum value, the 75th percentile, 
the median, and the mean value for each pattern across 
all of the tested spreadsheets. 
The results are shown in Table~\ref{tbl:exp_pattern_size}. 
We see that \rr and \ff patterns compress the most edges. 
\rr and \ff can reduce up to more than 500k and 200k edges, respectively. 
\rrChain and \rrGap can also reduce a significant number of edges 
(i.e., up to 24k and 19k respectively). 
While \rf and \fr do not reduce as many edges as the other patterns, 
we believe they are still prevalent in modern spreadsheets based on a recent survey of spreadsheet users~\cite{Antifreeze}.


==> fig/ex-copy.tex <==
% !TEX root = ../../thesis.tex
\begin{tikzpicture}
    \newcommand{\zsep}{1.3em}
    \newcommand{\xsep}{7.0em}
    \newcommand{\ysep}{1.4em}
    \newcommand{\wsep}{8.5em}
    \newcommand{\eps}{0.1em}
    \begin{scope}
        \fill[gray!30] (0.0,4*\ysep) rectangle (1*\xsep,5*\ysep);
        \fill[gray!30] (-\zsep,0*\ysep) rectangle (0.0,5*\ysep);
        % horizontal
        \foreach \x in {0,...,5} {
            \draw (-\zsep,\x*\ysep) -- (1*\xsep,\x*\ysep);
        }
        % vertical
        \foreach \x in {0,...,1} {
            \draw (\x*\xsep,0*\ysep) -- (\x*\xsep,5*\ysep);
        }
        \draw (-\zsep,0*\ysep) -- (-\zsep,5*\ysep);
        % row header
        \node[labelnode] (a0) at (0.5*\xsep,4.5*\ysep)  {\code{A}};
        % row 1
        \node[labelnode] (x1) at (-0.5*\zsep,3.5*\ysep)  {\code{1}};
        \node[cellnode,c_size_c,anchor=center] (a1) at (0.5*\xsep,3.5*\ysep)  {\formula{=SUM(\$C\$1:C1)}};
        % row 2
        \node[labelnode] (x2) at (-0.5*\zsep,2.5*\ysep)  {\code{2}};
        % row 3
        \node[labelnode] (x3) at (-0.5*\zsep,1.5*\ysep)  {\code{3}};
        % row 4
        \node[labelnode] (x4) at (-0.5*\zsep,0.5*\ysep)  {\code{4}};
        \node[cellnode,c_size_b,anchor=center] (a4) at (0.5*\xsep,0.5*\ysep)  {\formula{=SUM(\$C\$1:C4)}};
        \node[labelnode] (a0) at (0.5*\xsep,-0.5*\ysep)  {(a)};
        \draw[black,very thick]  (0*\xsep+\eps,0*\ysep+\eps) rectangle (1*\xsep-\eps,1*\ysep-\eps);
        \draw[black,dashed,thick] (0*\xsep+\eps,3*\ysep+\eps) rectangle (1*\xsep-\eps,4*\ysep-\eps);
        \fill[black]  (1*\xsep-3*\eps,0*\ysep-\eps) rectangle ++(4*\eps,4*\eps);
    \end{scope}
    \begin{scope}[xshift=2*\xsep]
        \fill[gray!30] (0.0,4*\ysep) rectangle (1*\xsep,5*\ysep);
        \fill[gray!30] (-\zsep,0*\ysep) rectangle (0.0,5*\ysep);
        % horizontal
        \foreach \x in {0,...,5} {
            \draw (-\zsep,\x*\ysep) -- (1*\xsep,\x*\ysep);
        }
        % vertical
        \foreach \x in {0,...,1} {
            \draw (\x*\xsep,0*\ysep) -- (\x*\xsep,5*\ysep);
        }
        \draw (-\zsep,0*\ysep) -- (-\zsep,5*\ysep);
        % row header
        \node[labelnode] (a0) at (0.5*\xsep,4.5*\ysep)  {\code{A}};
        % row 1
        \node[labelnode] (x1) at (-0.5*\zsep,3.5*\ysep)  {\code{1}};
        \node[cellnode,c_size_c,anchor=center] (a1) at (0.5*\xsep,3.5*\ysep)  {\formula{=SUM(\$C\$1:C1)}};
        % row 2
        \node[labelnode] (x2) at (-0.5*\zsep,2.5*\ysep)  {\code{2}};
        \node[cellnode,c_size_b,anchor=center] (a2) at (0.5*\xsep,2.5*\ysep)  {\formula{=SUM(\$C\$1:C2)}};
        % row 3
        \node[labelnode] (x3) at (-0.5*\zsep,1.5*\ysep)  {\code{3}};
        \node[cellnode,c_size_b,anchor=center] (a3) at (0.5*\xsep,1.5*\ysep)  {\formula{=SUM(\$C\$1:C3)}};
        % row 4
        \node[labelnode] (x4) at (-0.5*\zsep,0.5*\ysep)  {\code{4}};
        \node[cellnode,c_size_b,anchor=center] (a4) at (0.5*\xsep,0.5*\ysep)  {\formula{=SUM(\$C\$1:C4)}};
        \node[labelnode] (a0) at (0.5*\xsep,-0.5*\ysep)  {(b)};
        \draw[black,dashed,thick]
           (0*\xsep+\eps,3*\ysep-\eps)
        -- (0*\xsep+\eps,0*\ysep+\eps)
        -- (1*\xsep-\eps,0*\ysep+\eps)
        -- (1*\xsep-\eps,3*\ysep-\eps);
        \draw[black,very thick]    (0*\xsep+\eps,3*\ysep+\eps) rectangle (1*\xsep-\eps,4*\ysep-\eps);
        \fill[black]  (1*\xsep-3*\eps,3*\ysep-\eps) rectangle ++(4*\eps,4*\eps);
        \fill[black]  (1*\xsep-5*\eps,0*\ysep-0*\eps) rectangle ++(8*\eps,2*\eps);
        \fill[black]  (1*\xsep-2*\eps,0*\ysep-3*\eps) rectangle ++(2*\eps,8*\eps);
    \end{scope}
\end{tikzpicture}


==> fig/ex-edge-types.tex <==
% !TEX root = ../../thesis.tex
\begin{tikzpicture}
    \newcommand{\zsep}{6.0em}
    \newcommand{\xsep}{7.0em}
    \newcommand{\ysep}{1.4em}
    \newcommand{\wsep}{1.0em}
    \newcommand{\eps}{1.5em}
    \begin{scope}
        \node[depgraphnode] (a1) at (0*\xsep,-1*\ysep)  {\code{A1}};
        \node[depgraphnode] (a2) at (0*\xsep,-2*\ysep)  {\code{A2}};
        \node[depgraphnode] (a3) at (0*\xsep,-3*\ysep)  {\code{A3}};
        \node[depgraphnode] (a4) at (0*\xsep,-4*\ysep)  {\code{A4}};
        \node[depgraphnode] (a5) at (0*\xsep,-5*\ysep)  {\code{A5}};
        \node[depgraphnode] (b1) at (1*\xsep,-1*\ysep)  {\code{B1}};
        \node[depgraphnode] (b2) at (1*\xsep,-2*\ysep)  {\code{B2}};
        \node[depgraphnode] (b3) at (1*\xsep,-3*\ysep)  {\code{B3}};
        \draw[depgraphedge] (a1) -- (b1);
        \draw[depgraphedge] (a2) -- (b1);
        \draw[depgraphedge] (a2) -- (b2);
        \draw[depgraphedge] (a3) -- (b1);
        \draw[depgraphedge] (a3) -- (b2);
        \draw[depgraphedge] (a3) -- (b3);
        \draw[depgraphedge] (a4) -- (b2);
        \draw[depgraphedge] (a4) -- (b3);
        \draw[depgraphedge] (a5) -- (b3);
        \node[depgraphnode] (aa) at (0*\xsep,-8*\ysep)  {\code{A1:A5}};
        \node[depgraphnode] (bb) at (1*\xsep,-8*\ysep)  {\code{B1:B3}};
        \draw[depgraphedge] (aa) -- node[above]{$\mathrm{MM}(\code{A1},3)$} (bb);
        \node[right of=b1,node distance=1em,labelnode,anchor=west] (lb1) {ref to \code{A1:A3}};
        \node[right of=b2,node distance=1em,labelnode,anchor=west] (lb2) {ref to \code{A2:A4}};
        \node[right of=b3,node distance=1em,labelnode,anchor=west] (lb3) {ref to \code{A3:A5}};
        \draw (0*\xsep-\wsep-\eps,-5*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-1*\ysep+\eps);
        \draw (0*\xsep-\wsep-\eps,-8*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-8*\ysep+\eps);
        \node[labelnode] (eq) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-6.5*\ysep)  {$=$};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep)  {(a) Moving-beginning Moving-ending};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep-1em) {``sliding window''};
    \end{scope}
    \begin{scope}[xshift=2.8*\xsep]
        \node[depgraphnode] (a1) at (0*\xsep,-1*\ysep)  {\code{A1}};
        \node[depgraphnode] (a2) at (0*\xsep,-2*\ysep)  {\code{A2}};
        \node[depgraphnode] (a3) at (0*\xsep,-3*\ysep)  {\code{A3}};
        \node[depgraphnode] (a4) at (0*\xsep,-4*\ysep)  {\code{A4}};
        \node[depgraphnode] (a5) at (0*\xsep,-5*\ysep)  {\code{A5}};
        \node[depgraphnode] (b1) at (1*\xsep,-1*\ysep)  {\code{B1}};
        \node[depgraphnode] (b2) at (1*\xsep,-2*\ysep)  {\code{B2}};
        \node[depgraphnode] (b3) at (1*\xsep,-3*\ysep)  {\code{B3}};
        \node[depgraphnode] (b4) at (1*\xsep,-4*\ysep)  {\code{B4}};
        \node[depgraphnode] (b5) at (1*\xsep,-5*\ysep)  {\code{B5}};
        \draw[depgraphedge] (a1) -- (b1);
        \draw[depgraphedge] (a1) -- (b2);
        \draw[depgraphedge] (a1) -- (b3);
        \draw[depgraphedge] (a1) -- (b4);
        \draw[depgraphedge] (a1) -- (b5);
        \draw[depgraphedge] (a2) -- (b2);
        \draw[depgraphedge] (a2) -- (b3);
        \draw[depgraphedge] (a2) -- (b4);
        \draw[depgraphedge] (a2) -- (b5);
        \draw[depgraphedge] (a3) -- (b3);
        \draw[depgraphedge] (a3) -- (b4);
        \draw[depgraphedge] (a3) -- (b5);
        \draw[depgraphedge] (a4) -- (b4);
        \draw[depgraphedge] (a4) -- (b5);
        \draw[depgraphedge] (a5) -- (b5);
        \node[depgraphnode] (aa) at (0*\xsep,-8*\ysep)  {\code{A1:A5}};
        \node[depgraphnode] (bb) at (1*\xsep,-8*\ysep)  {\code{B1:B5}};
        \draw[depgraphedge] (aa) -- node[above]{$\mathrm{SM}(\code{A1},5)$} (bb);
        \node[right of=b1,node distance=1em,labelnode,anchor=west] (lb1) {ref to \code{A\$1:A1}};
        \node[right of=b2,node distance=1em,labelnode,anchor=west] (lb2) {ref to \code{A\$1:A2}};
        \node[right of=b3,node distance=1em,labelnode,anchor=west] (lb3) {ref to \code{A\$1:A3}};
        \node[right of=b4,node distance=1em,labelnode,anchor=west] (lb4) {ref to \code{A\$1:A4}};
        \node[right of=b5,node distance=1em,labelnode,anchor=west] (lb5) {ref to \code{A\$1:A5}};
        \draw (0*\xsep-\wsep-\eps,-5*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-1*\ysep+\eps);
        \draw (0*\xsep-\wsep-\eps,-8*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-8*\ysep+\eps);
        \node[labelnode] (eq) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-6.5*\ysep)  {$=$};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep) {(b) Stationary-beginning Moving-ending};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep-1em) {``expanding window''};
    \end{scope}
    \begin{scope}[yshift=-13*\ysep]
        \node[depgraphnode] (a1) at (0*\xsep,-1*\ysep)  {\code{A1}};
        \node[depgraphnode] (a2) at (0*\xsep,-2*\ysep)  {\code{A2}};
        \node[depgraphnode] (a3) at (0*\xsep,-3*\ysep)  {\code{A3}};
        \node[depgraphnode] (a4) at (0*\xsep,-4*\ysep)  {\code{A4}};
        \node[depgraphnode] (a5) at (0*\xsep,-5*\ysep)  {\code{A5}};
        \node[depgraphnode] (b1) at (1*\xsep,-1*\ysep)  {\code{B1}};
        \node[depgraphnode] (b2) at (1*\xsep,-2*\ysep)  {\code{B2}};
        \node[depgraphnode] (b3) at (1*\xsep,-3*\ysep)  {\code{B3}};
        \node[depgraphnode] (b4) at (1*\xsep,-4*\ysep)  {\code{B4}};
        \node[depgraphnode] (b5) at (1*\xsep,-5*\ysep)  {\code{B5}};
        \draw[depgraphedge] (a1) -- (b1);
        \draw[depgraphedge] (a2) -- (b1);
        \draw[depgraphedge] (a2) -- (b2);
        \draw[depgraphedge] (a3) -- (b1);
        \draw[depgraphedge] (a3) -- (b2);
        \draw[depgraphedge] (a3) -- (b3);
        \draw[depgraphedge] (a4) -- (b1);
        \draw[depgraphedge] (a4) -- (b2);
        \draw[depgraphedge] (a4) -- (b3);
        \draw[depgraphedge] (a4) -- (b4);
        \draw[depgraphedge] (a5) -- (b1);
        \draw[depgraphedge] (a5) -- (b2);
        \draw[depgraphedge] (a5) -- (b3);
        \draw[depgraphedge] (a5) -- (b4);
        \draw[depgraphedge] (a5) -- (b5);
        \node[depgraphnode] (aa) at (0*\xsep,-8*\ysep)  {\code{A1:A5}};
        \node[depgraphnode] (bb) at (1*\xsep,-8*\ysep)  {\code{B1:B5}};
        \draw[depgraphedge] (aa) -- node[above]{$\mathrm{MS}(\code{A1},1)$} (bb);
        \node[right of=b1,node distance=1em,labelnode,anchor=west] (lb1) {ref to \code{A1:A\$5}};
        \node[right of=b2,node distance=1em,labelnode,anchor=west] (lb2) {ref to \code{A2:A\$5}};
        \node[right of=b3,node distance=1em,labelnode,anchor=west] (lb3) {ref to \code{A3:A\$5}};
        \node[right of=b4,node distance=1em,labelnode,anchor=west] (lb4) {ref to \code{A4:A\$5}};
        \node[right of=b5,node distance=1em,labelnode,anchor=west] (lb5) {ref to \code{A5:A\$5}};
        \draw (0*\xsep-\wsep-\eps,-5*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-1*\ysep+\eps);
        \draw (0*\xsep-\wsep-\eps,-8*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-8*\ysep+\eps);
        \node[labelnode] (eq) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-6.5*\ysep)  {$=$};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep)  {(c) Moving-beginning Stationary-ending};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep-1em) {``shrinking window''};
    \end{scope}
    \begin{scope}[xshift=2.8*\xsep , yshift=-13*\ysep]
        \node[depgraphnode] (a1) at (0*\xsep,-1*\ysep)  {\code{A1}};
        \node[depgraphnode] (a2) at (0*\xsep,-2*\ysep)  {\code{A2}};
        \node[depgraphnode] (a3) at (0*\xsep,-3*\ysep)  {\code{A3}};
        \node[depgraphnode] (b1) at (1*\xsep,-1*\ysep)  {\code{B1}};
        \node[depgraphnode] (b2) at (1*\xsep,-2*\ysep)  {\code{B2}};
        \node[depgraphnode] (b3) at (1*\xsep,-3*\ysep)  {\code{B3}};
        \node[depgraphnode] (b4) at (1*\xsep,-4*\ysep)  {\code{B4}};
        \node[depgraphnode] (b5) at (1*\xsep,-5*\ysep)  {\code{B5}};
        \draw[depgraphedge] (a1) -- (b1);
        \draw[depgraphedge] (a1) -- (b2);
        \draw[depgraphedge] (a1) -- (b3);
        \draw[depgraphedge] (a1) -- (b4);
        \draw[depgraphedge] (a1) -- (b5);
        \draw[depgraphedge] (a2) -- (b1);
        \draw[depgraphedge] (a2) -- (b2);
        \draw[depgraphedge] (a2) -- (b3);
        \draw[depgraphedge] (a2) -- (b4);
        \draw[depgraphedge] (a2) -- (b5);
        \draw[depgraphedge] (a3) -- (b1);
        \draw[depgraphedge] (a3) -- (b2);
        \draw[depgraphedge] (a3) -- (b3);
        \draw[depgraphedge] (a3) -- (b4);
        \draw[depgraphedge] (a3) -- (b5);
        \node[depgraphnode] (aa) at (0*\xsep,-8*\ysep)  {\code{A1:A3}};
        \node[depgraphnode] (bb) at (1*\xsep,-8*\ysep)  {\code{B1:B5}};
        \draw[depgraphedge] (aa) -- node[above]{$\mathrm{SS}(\code{A1},3)$} (bb);
        \node[right of=b1,node distance=1em,labelnode,anchor=west] (lb1) {ref to \code{A\$1:A\$3}};
        \node[right of=b2,node distance=1em,labelnode,anchor=west] (lb2) {ref to \code{A\$1:A\$3}};
        \node[right of=b3,node distance=1em,labelnode,anchor=west] (lb3) {ref to \code{A\$1:A\$3}};
        \node[right of=b4,node distance=1em,labelnode,anchor=west] (lb4) {ref to \code{A\$1:A\$3}};
        \node[right of=b5,node distance=1em,labelnode,anchor=west] (lb5) {ref to \code{A\$1:A\$3}};
        \draw (0*\xsep-\wsep-\eps,-5*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-1*\ysep+\eps);
        \draw (0*\xsep-\wsep-\eps,-8*\ysep-\eps) rectangle (1*\xsep+\zsep+\eps,-8*\ysep+\eps);
        \node[labelnode] (eq) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-6.5*\ysep)  {$=$};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep)  {(d) Stationary-beginning Stationary-ending};
        \node[labelnode] (a0) at (0.5*\xsep-0.5*\wsep+0.5*\zsep,-10*\ysep-1em) {``fixed window''};
    \end{scope}
\end{tikzpicture}


==> revision.tex <==
%!TEX root = paper.tex

\noindent {\large \bf Summary for Revised Paper \#849 
``Efficient and Compact Spreadsheet Formula Graphs''}

\vspace{1mm}

We thank the reviewers and meta-reviewer for their 
careful review of our paper and their helpful comments. 
We have thoroughly revised the paper based on their suggestions. 
We first summarize the major changes 
and then discuss the detailed changes for each review one by one. 
To aid the review of our changed text in the main paper, 
we have highlighted major text revisions using \rtwo{blue font}, 
added line numbers, and used \fpointer{x}{y}{z} to refer to 
a given line in the revised paper. 
We have made the following major changes:
\begin{itemize}
    \item We included a clearer explanation of the motivating applications, the significance of the problem, the overall goal of this paper, and the challenges for solving this problem in the introduction (\textbf{R1.O1, R3.\{O1,O2,O4\}}).
    
    \item We have more clearly described why the basic patterns are prevalent in Sec.~\ref{sec:basic_patterns} (\textbf{R2.O1}).
    
    \item We added a description for the \sys framework 
    in Sec.~\ref{sec:sys} (\textbf{R2.O2}).
    
    \item We added hardness proofs 
    for \rr, \rf, and \fr in Sec.~\ref{sec:sys} (\textbf{R1.D4}).
    
    \item We added a discussion on the limitations of the patterns in \sys and possible methods for extending these patterns or exploiting 
    other information for further compressing formula graphs in Sec.~\ref{sec:extension} (\textbf{R1.\{O3,D5\}, R2.O1}).
    
    \item We added a discussion on how the techniques of \sys 
    help spreadsheet users. We also added a link to an Excel plug-in that leverages \sys to help Excel users trace formula dependencies, 
    which is one of our use cases, in Sec.~\ref{sec:exp} (\textbf{R3.\{O1,O4\}}).
    
    \item We added experiments for comparing \sys with 
    a baseline that leverages RedisGraph to store, query, and maintain formula graphs (Fig.~\ref{fig:exp_antifreeze_build}-\ref{fig:exp_antifreeze_modify}) 
    and an approach derived from OpenOffice Calc (Fig.~\ref{fig:exp_excel}) in Sec.~\ref{sec:exp} (\textbf{R1.\{O2,O4\}}).
\end{itemize}

\subsection*{\bf Reviewer \#1}

\Rev{O1}{What exactly is the motivation? Speeding up chart update in spreadsheets seems like a nice idea, but is there a need in industry for instant chart update? Is the problem so big and challenging? What is the overall goal? To optimize opening time of a file?
It would be nice if the authors can provide a concrete example of a use case that would greatly benefit from the time advantage offered by their dependent finding algorithm. It seems that they can reduce the time of a $>1$ minute chart update to $<0.5$ seconds, but adding a paragraph on how that can help someone achieve their work faster would be great.}

\Ans{We believe reducing the latency for 
finding dependents and precedents 
in a spreadsheet formula graph is a big and important problem because 
i) spreadsheets are adopted by many users (i.e., 1 billion users) 
across different domains; ii) querying a formula graph 
in large and complex real-world spreadsheets 
often leads to a long response time; and 
iii) a larger latency during data analysis 
significantly hinders data exploration process. 
For example, our experiments in Sec.~\ref{sec:exp} show that 
using a baseline approach to find dependents in a formula graph 
can take up to 49 seconds for real spreadsheets, 
while our techniques reduce it to 3~ms. 
A previous study on the effects of latency 
on data exploration has shown that even an additional delay of 
just 0.5 seconds ``results in reduced interaction and reduced 
dataset coverage during analysis''~\cite{Latency_LiuH14}, 
with fewer hypotheses explored and insights generated. 
A more than 48 seconds ($>99\%$) reduction in latency can be a huge boost 
for end-users' exploration, experimentation, and insight discovery.

There are two major applications that are supported 
by finding dependents/precedents and require interactive speeds. 
First, accelerating finding dependents in a formula graph 
does not only speed up updating a spreadsheet, 
but also more quickly return control to the user 
under an asynchronous execution model~\cite{Antifreeze}. 
Specifically, when a cell is updated, 
the spreadsheet system will query the formula graph to 
find the formulae that need recalculation, 
mark the corresponding cells as invisible, 
and return control to the user such that the user can interact with 
the visible cells. The system will then recalculate 
the new results of the invisible formulae in the background. 
In this scenario, finding dependents is on the critical path 
for returning control to the user and is therefore critical 
in ensuring interactivity. 

Another application is formula 
dependency visualization. Existing spreadsheet systems provide 
tools for users to find and visualize the dependents or precedents 
of cells to help users check the accuracy of formulae 
and identify sources of errors, which spreadsheets are known 
to have a lot of~\cite{spreadsheetError, spreadsheetHorrorStory}. 
This application also requires querying the formula graph interactively.
To demonstrate this application, 
we have implemented a plug-in in Excel that leverages \sys to 
quickly find and visualize dependents/precedents. 
We have prepared a demo video that shows how the plug-in works 
(\url{https://youtu.be/qxZWVJ7THjw}). 
%Overall, debugging spreadsheet formula graphs requires \sys 
%for interactivity.

Therefore, the overall goal of \sys is to reduce the execution 
time for finding dependents/precedents in a formula graph and 
thereby efficiently support the aforementioned applications. 

In the revised paper, we now more clearly 
discuss the motivating applications (\fpointer{1}{1}{33}), 
the significance of this problem we consider (\fpointer{1}{2}{66}), 
and the overall goal of this paper (\fpointer{1}{2}{74}) in Sec.~1.

Regarding why this problem is challenging, 
in our original paper, we discussed three challenges 
for solving this problem, 
including: i) spreadsheets are complex and a formula could include 
multiple references to different rows or columns, making identifying 
the common patterns across formulae difficult; 
ii) we need to develop novel algorithms 
for directly querying the compressed formula 
graph without decompressing it; 
and iii) the compressed formula graph requires 
incremental maintenance for interactivity. 
In the revised paper, we now more clearly highlight the challenges 
in Sec.~1 (\fpointer{2}{1}{97}).
}

\Rev{O2}{It would also be nice if they tested their algorithm against another common business spreadsheet viewer, that is open source – like LibreOffice / OpenOffice. That way, they could be able to compare better against them, as Excel is a blackbox and they are not able to separate the time to find dependents from the time to execution, of a chart update as well.}

\Ans{Unlike Excel, 
Libre/OpenOffice Calc does not provide an API 
for finding dependents and precedents, nor 
does it provide easy hooks within its source code to do so. 
So, we cannot directly 
evaluate the performance of finding dependents and precedents 
in Calc. Instead, we implemented a new baseline, \calc, 
based on a document that describes 
the design of formula graphs in OpenOffice Calc~\cite{calc-dep-graph}. 
Similar to \nocomp, this baseline does not compress dependencies. 
The only difference from \nocomp is that 
it adopts a customized data structure 
to find the vertices in formula graphs 
that overlap with an input range, 
rather than using an R-Tree. \calc partitions 
the full spreadsheet space (i.e., 1,048,576, or $2^{20}$,  
rows and 16,384 columns) 
into pre-defined ranges, where each range is represented by 
a container. A vertex is put into a container 
if this vertex overlaps with 
this container's represented range. 
\calc evenly partitions the column space, 
with the number of columns in each container equal to 256. 
On the row dimension, for the rows between 1 and $2^{15}$ 
each container has 256 rows, 
and for the rest of the rows (i.e., from row $2^{15}$ to $2^{20}$)  
each container has 128 rows. 
The containers for the upper part of a spreadsheet have more 
rows since the upper part is more likely to 
be referenced by formulae. 

We added an experiment to compare \calc with \sys. 
Among the 20 spreadsheets we have tested, \calc cannot 
finish finding dependents within 300 seconds in 2 spreadsheets. 
For the spreadsheets where \calc can finish, \sys is much 
faster than \calc on finding dependents in all cases. 
The speedup of \sys over \calc is up to 1,682$\times$. 
The experiment setup and results 
are added to Sec.~\ref{sec:exp_commercial} (\fpointer{12}{1}{991}).
}

\Rev{O3}{Tabular locality is stressed but it is only used in the greedy approach to find the candidate edges for a new edge to merge. Is it only adjacent relationship considered? What about other types of locality like the row or column locality, the type of formula, etc.}

\Ans{In its current design, \sys supports patterns 
in formula cells that are adjacent along the column and row axis. 
Therefore, \sys \textit{does} support row and column locality 
for adjacent formula cells. 
\sys is focused on the patterns in adjacent formula cells 
since these relationships are prevalent in 
real spreadsheets. Indeed, this alone is sufficient for a significant 
reduction in the execution time for finding dependents, 
as shown in our experiments. 

However, the patterns we consider in \sys 
represent a subset of tabular locality in spreadsheets. 
It is possible to extend these patterns or 
exploit other patterns to further 
reduce the sizes of formula graphs. 
For example, one extended pattern derived from \rr could be 
that the referenced ranges in the formula cells 
of every other row follow the \rr pattern (denoted as \rrGapOne).  
We have now tested its prevalence 
and found it is much less prevalent than its \rr counterpart. 
Specifically, \rrGapOne reduces the number of edges by 195k 
and 275k for Enron and Github datasets, respectively, while 
the number of edged reduced by \rr for the two datasets 
is 17.4M and 141.9M, respectively. 
It is also possible to exploit other information, 
such as a column of formulae having the same functions, 
to better compress formula graphs. 
Fully exploiting these patterns and information is left to future work. 
That said, we would like to point out that a more
complex compressed representation that leverages 
more advanced forms of locality, 
while leading to smaller formula graphs, 
could be expensive to build and incrementally maintain. 
We believe the space of patterns we support offer a suitable trade-off 
between compression ratios and interactivity.
We have now added a discussion for the limitations of 
the patterns supported by \sys and how to extend these patterns 
in Sec.~\ref{sec:extension} (\fpointer{9}{1}{768}).
}

%We did not consider the patterns 
%that go beyond the adjacent relationships, 
%such as the repeated patterns with a fixed gap, 
%since we found these patterns are 
%not helpful in reducing the execution time for finding dependents. 
%The reason is that finding the dependents of a range of cells in 
%an edge that is compressed by these patterns 
%will return multiple separate ranges or cells, 
%which essentially decompresses the edge. 
%So, the complexity of finding dependents 
%becomes $O(\text{the number of compressed dependencies})$ 
%rather than $O(1)$, as in the patterns that 
%consider adjacent relationships. 
%Consider the example where 
%the formulae in cells \code{B1}, \code{B3}, and \code{B5} 
%are \code{A1+1}, \code{A3+1}, and \code{A5+1}, respectively, 
%and B2 and B4 only include pure values. 
%We can leverage \rr to compress these dependencies with 
%the gap information included 
%(i.e., $\code{A1:A5} \rightarrow \code{B1:B5}$ and the gap is 1). 
%If we need to find the dependents of \code{A1:A5}, 
%the returned results will be \code{B1}, \code{B3}, \code{B5}. 
%
%However, we agree that the patterns considered 
%in the paper cover a portion of the tabular locality 
%in spreadsheets. It is possible to further leverage other 
%information, such as the same formula function in a column, 
%to better compress the formula graph, which is left to future work. 
%In Section~\ref{sec:extension} of our revised paper, 
%we now clarified these points at \fpointer{}{}{}. 


\Rev{O4}{I am not sure why don’t you test with an in-mem graph db (Redis graph or any other alternative) as well? The NoComp alternative is a simple (naive) alternative. I expect that for large graphs the graph DBs exploits the custom indexes for these types of queries and maybe fast enough for your requirements.}

\Ans{We have implemented a new baseline that leverages \redis 
to store, query, and maintain formula graphs. 
Since \redis and other existing graph databases do not 
consider the range characteristics of spreadsheets 
or support finding the overlapping vertices for an input range, 
we have to decompose each edge that involves a range 
in the original uncompressed formula graph 
into multiple edges that only involve cells. 
For example, an edge $\code{A1:A2} \rightarrow \code{B1}$ 
is decomposed into two edges $\code{A1} \rightarrow \code{B1}$ 
and $\code{A2} \rightarrow \code{B1}$. 
To efficiently load a formula graph in \redis, we 
write these decomposed edges into a CSV file and adopt 
\redis's bulk-load tool to load the CSV file into the database 
rather than inserting each edge one by one. 
We use Cypher, a declarative graph query language, 
to query and maintain the graph. 

Our new experiments in Sec.~\ref{sec:exp_antifreeze} 
(\fpointer{11}{1}{941}) 
show that \redis cannot finish loading the graph within 
300 seconds in two cases because the formula graph that only 
includes cell-to-cell edges is too large. 
We have observed a case where the CSV file that stores 
the decomposed edges is as large as 3.5 GB. 
In addition, finding dependents \redis 
cannot finish within 60 seconds in many cases due to large graphs. 
Among the tests where \redis can finish, 
\sys has much smaller execution time than \redis 
in most of these tests. The speedup of \sys over \redis 
for finding dependents is up to 19,555$\times$.}

\Rev{D1}{There is one email more (7) that the number of authors (6). Either there is an author missing or the email srinivasan.seshadri@berkeley.edu is not needed.}

\Ans{We have added the missing author name in the paper. 
Note that we did not change the author list in the CMT system.}

\Rev{D2}{The use of CDF in the intro is not the most appropriate. I would prefer a plain distribution and see what the majority of the spreadsheets has.}

\Ans{We have now refactored Figure~\ref{fig:num_dependents} to 
plot probability distributions 
for the maximum number of dependents and the longest 
path in the Enron and Github datasets.}

\Rev{D3}{Problem statement. You mention that ``...the time for maintaining G with respect to the updates is small...'' This is a bit vague, Can you provide a better formulation wrt G’? E.g., is smaller or equal or at the same scale of updates on G’?}

\Ans{We have refactored the sentence ``...the time for maintaining 
$G$ with respect to the updates is small...'' 
to ``...the time for maintaining $G$ is also 
smaller than the time for maintaining $G^\prime$  
with respect to the same updates...'' (\fpointer{3}{2}{273}).}

\Rev{D4}{Theorem 1. Mention how RR,RF,FR are reduced also in RPC.}

\Ans{We now have additionally reduced 
the rectilinear picture compression (RPC) problem 
to the compressed edge minimization (CEM) problem 
if we consider \rr, \rf, and \fr, respectively (\fpointer{6}{2}{547}). 
Note, however, that since CEM includes all of \rr, \rf, \fr, and \ff,
we have already shown that CEM is NP hard.
Now we demonstrate that CEM(\rr), CEM(\fr), and CEM(\fr), 
subsets of the problem restricted to those types of formulae, 
are still NP hard.

Recall that RPC is defined as finding the minimal number 
of rectangles that precisely cover 1's in a $m\times n$ matrix 
that only has 1's and 0's. To reduce RPC to CEM,  
we map the input matrix to a spreadsheet range $R$: 
for each value at column $i$ and row $j$ in the matrix, 
if the value is 1, we place a formula at $(i, j)$ in $R$; 
otherwise, we place a pure value at $(i, j)$ in $R$. 
If the dependencies of any range of formulae in $R$ 
can be compressed into a single edge by a pattern $p$, then 
the RPC problem is equivalent to minimizing the number of 
edges of the compressed graph $G$ for $R$ if we only consider 
the pattern $p$. 

Therefore, we need to construct a range $R$ for each pattern $p$ 
such that the dependencies of any range of formulae in $R$ 
can be compressed into a single edge by $p$. 
For \ff, we let all of the formulae in $R$ 
reference the same fixed range outside $R$ to 
meet the above condition. 
Similarly, for \rr, we let each formula in $R$ 
reference the cell to its left. 
For \rf, we first construct another range $R^\prime$ 
that can be compressed into a single edge by \rf 
and has the same shape as $R$. 
Note that in $R^\prime$, the dependencies of any range of formulae 
can also be compressed into a single edge by \rf. 
For example, assuming $R^\prime = (\code{B1:C3})$, 
where the formulae in the first column is 
$\code{SUM(A1:A1)}, \code{SUM(A2:A1), \code{SUM(A3:A1)}}$ 
and the formulae in the second column is 
$\code{SUM(B1:A1)}, \code{SUM(B2:A1), \code{SUM(B3:A1)}}$. 
Here, the dependencies in these formulae follow the \rf pattern 
since the head cell of each referenced range is relative 
(i.e., \code{A1} for the formula cell \code{B1}, 
\code{A2} for \code{B2}, and so on) 
while the tail cell is fixed (i.e., \code{A1}). 
After we construct $R^\prime$, we generate $R$ by 
copying the formula at $(i, j)$ in $R^\prime$ 
to $(i, j)$ in $R$ if the cell $(i, j)$ in $R$ is a formula cell. 
This way, we construct a range $R$ where the dependencies 
of any range of formulae in $R$ can be compressed into a single 
edge by \rf. The \fr case is done symmetrically. 
}

\Rev{D5}{The support of an additional pattern (RR-Chain) makes me wonder whether all patterns (4+1) cover all possible combinations of formulas and how efficiently this is performed with the greedy algo, especially when cells are not in consecutive cell ranges.
For example, can you please clarify the following? 
if you have the following rules
\{B1=A1+constant, B3=A3+constant, B5=A5+constant, $\cdots$ (odd cells) $\cdots$ up to Bn-1=An-1+constant\} and
\{C2 =A2+constant2, C4 =A4+constant, $\cdots$ (even cells) $\cdots$ 
up to Cn=An+constant\}. 
How many compressed edges are you going to produce? (A1:An-1) $\rightarrow$ (B1,Bn-1) is not accurate since it contains the even cells which are captured by another rule. (A2:An) $\rightarrow$ (C2,Cn).
}

\Ans{As mentioned in the response to \textbf{R1.O3}, 
the basic patterns along with the extended one focus 
on patterns for adjacent formula cells, which are 
prevalent in real spreadsheets and effective in 
reducing the time for finding dependents. 
Therefore, for the example mentioned in the comment, 
the current design of \sys do not compress them 
since the patterns in both column \code{B} and \code{C} 
are repeated with a fixed gap. 
However, it is possible to extend \rr pattern that 
consider a fixed gap to compress the two columns of formulae, 
which is called \rrGapOne. 
Fully exploiting other patterns and information in spreadsheets 
is left to future work. 
We have now added a discussion for the limitations of 
the patterns supported by \sys and how to extend these patterns 
in Sec.~\ref{sec:extension} (\fpointer{9}{1}{768}).
}

%However, as discussed in the response to \textbf{R1.O3}, 
%we do not consider these patterns because they 
%are not helpful 
%in reducing the execution time for finding dependents. 
%We also note that it is possible to leverage 
%other information related to tabular locality to better 
%compress formula graphs. 
%Please find the details in the response to \textbf{R1.O3}. 
%We have now clarified the above points at \fpointer{1}{2}{3}.


\Rev{D6}{Exps section . Comparison with NoComp. It is not clear to me. In both Taco and NoComp, finding immediate dependents should be an O(1) task.}

\Ans{In the experiment section and also in this paper, when we say ``find dependents'', we mean ``find both direct and indirect dependents''. Therefore, the complexity for finding dependents 
is not O(1) and should be the one summarized in  Table~\ref{tbl:complexity} (\textcolor{purple}{page 8}). 
We have added one 
sentence to clarify this point in Sec.~\ref{sec:exp_nocomp}  (\fpointer{10}{2}{908}).}

\Rev{Inclusive Writing}{Bars in bar charts, could also include shapes to differentiate them instead of only colors.}

\Ans{We have now included shapes in the bar charts (i.e., 
Fig.~\ref{fig:num_dependents} and Fig.~\ref{fig:exp_antifreeze_build}-\ref{fig:exp_excel}).} 

\subsection*{\bf Reviewer \#2}
\Rev{O1}{The descriptive power of the basic patterns is a bit unclear. It is hard to tell how well the current design can cover real-world spreadsheet formula dependencies. Does it always succeed? Or there is a limitation in certain scenarios. The ``applicability of basic patterns'' section briefly discussed it but not enough.}

\Ans{We have now more thoroughly discussed the applicability 
of the basic patterns at \fpointer{4}{2}{359} 
and added a discussion for the limitations of the patterns 
\sys supports in Sec.~\ref{sec:extension} (\fpointer{9}{1}{768}). 

One major reason why the basic patterns are prevalent 
in real spreadsheets is that modern spreadsheet systems 
(e.g., Excel, Google Sheets, and LibreOffice Calc)
provide a tool, called autofill, to help users generate 
a large number of formulae automatically, 
and the patterns adopted by autofill end up being the basic patterns. 
Specifically, autofill generates formulae by 
applying the pattern of one source formula cell to adjacent cells. 
For the generated formulae, the formula functions (e.g., \code{SUM}) 
are the same as in the source cell, but the references 
(e.g., \code{A1:B1}) are modified based on the following rules: 
if a reference is prefixed 
with a dollar sign \texttt{\$}, it is a fixed reference; 
otherwise it is a relative reference. 
Therefore, if a range $R$ in the source cell 
does not have \texttt{\$}, 
the generated ranges from $R$ follow the \rr pattern. 
If $R$'s head cell does not have \texttt{\$} but the tail cell does, 
the generated ranges follow \rf. 
The \fr pattern is generated symmetrically. 
Finally, if $R$'s tail and head cells have \texttt{\$}, 
the generated ranges follow \ff. 
But a formula may mix many ranges and include outliers, 
which makes extracting basic patterns from these formulae challenging. 

While there are other methods for generating formula cells 
(e.g., programmatically), we believe these methods are still likely to 
generate the basic patterns 
since these patterns are the building blocks for many applications, 
as discussed in the original paper. 
In fact, our experiments in Sec.~\ref{sec:exp_graph_size} 
show that leveraging the basic patterns 
in Sec.~\ref{sec:extension} reduce the number of 
edges of formula graphs for two real spreadsheet datasets 
to 5\% and 1.9\%, respectively, which shows that the 
basic patterns are prevalent in real spreadsheets.

The limitation of the basic patterns is that they 
focus on the patterns in adjacent formula cells along 
both column and row axis. So, they only 
represent a subset of tabular locality in spreadsheets. 
However, it is possible to extend these patterns or 
exploit other patterns to further 
reduce the sizes of formula graphs. 
For example, one extended pattern derived from \rr could be 
that the referenced ranges in the formula cells 
of every other row follow the \rr pattern (denoted as \rrGapOne).  
We have now tested its prevalence 
and found it is much less prevalent than its adjacent counterpart. 
Specifically, \rrGapOne reduces the number of edges by 195k 
and 275k for Enron and Github datasets, respectively, while 
the number of edged reduced by \rr for the two datasets 
is 17.4M and 141.9M, respectively. 
It is also possible to exploit other information, 
such as a column of formulae having the same functions, 
to better compress formula graphs. 
Fully exploiting these patterns and information is left to future work. 
}

\Rev{O2}{The ``TACO framework'' was mentioned in the introduction section in p2 but it would be better to give a more detailed definition/description about the TACO framework in Section IV for completeness and better clarity.}

\Ans{We have now more clearly described the \sys framework at the beginning of Sec.~\ref{sec:sys} (\fpointer{6}{1}{518}). 
Specifically, the \sys framework includes four generic 
and extensible algorithms 
for efficiently compressing, querying, 
and modifying formula graphs. 
These algorithms are extensible since 
they only utilize the four key functions for a pattern 
as shown in Sec.~\ref{sec:keyfunctions} 
and a pattern can be integrated into the \sys framework 
if they implement these functions.}

\Rev{O3}{The titles of some subsections in Section VI (e.g., ``Comparison with NoComp'') are not quite informative and self-explanatory.}

\Ans{We have modified the titles for Sec.~\ref{sec:exp_nocomp}, 
Sec.~\ref{sec:exp_antifreeze}, and Sec.~\ref{sec:exp_commercial} 
to be ``Performance Comparison with \nocomp'', 
``Performance Comparison with \anti and \redis '', and 
``Performance Comparison with Excel and \calc'', respectively. 
}

\Rev{D1}{“NoComp” is defined in p4 but mentioned in p3.}

\Ans{In the original paper, we used ``NoComp'' 
to represent both the pattern for an uncompressed edge 
in the compressed graph by \sys and the approach that does not 
compress formula graphs. 
The ``NoComp'' mentioned in p3 represents the pattern 
for an uncompressed edge. 

To clear up the confusion, in the revised paper, 
we now use ``\ncPattern'' to represent 
the pattern for an uncompressed edge in the graph 
compressed by \sys and clearly defined \ncPattern 
when it is first mentioned at \fpointer{3}{2}{264}. 
}

\subsection*{\bf Reviewer \#3}

\Rev{O1}{Spreadsheets have 1 billions users, but they mainly use Microsoft Excel. How many active users of DataSpread?}

\Ans{A version of Dataspread has been used by dozens to hundreds of 
users for processing genomics data, part of a 
National Institutes of Health 
sponsored genomics center, called KnowEng. 

However, improving the performance of Dataspread alone is not 
the focus of this paper. 
The algorithms of \sys are general-purpose 
and independent of the specific implementation of a spreadsheet system 
and can be integrated into any spreadsheet system to 
accelerate formula recalculation 
and reduce the time for returning control to the user. 

In addition, the \sys library can also be used to 
trace formula dependencies without requiring modifications 
to the internals of the spreadsheet system. 
Existing spreadsheet tools provide 
tools for users to find and visualize the dependents 
and precedents of cells 
to help users check the accuracy of formulae and 
identify sources of errors, 
which requires querying the formula graph interactively. 
We have implemented a plug-in in Excel that leverages \sys 
to quickly trace formula dependencies.  
We have prepared a demo video 
that shows how the plug-in works (\url{https://youtu.be/qxZWVJ7THjw}). 

More broadly speaking, we believe the research on spreadsheets 
should not be restricted to industry (e.g., Microsoft Excel 
or Google Sheets) but should also be pursued by academia. 
Our previous paper on benchmarking modern modern spreadsheet 
systems has shown many performance issues that need to 
be addressed for processing large datasets 
in spreadsheets~\cite{Benchmark_RahmanMBZKP20}. 
We have discussed these issues with the Google Sheets team. 
Such dialogues can lead to synergistic improvements in popular tools. 

In the revised paper, we have now more clearly explained 
the applications supported by formula graphs in 
the introduction (\fpointer{1}{1}{33}) and 
how the techniques of \sys can be adopted to help 
spreadsheet users in Sec.~\ref{sec:benchmark_config} (\fpointer{9}{2}{809}).}

\Rev{O2}{Is it a hard problem? Taking Section IV for example, any ``reasonable heuristic'' can significantly reduce the graph space and improve the efficiency. Technically, the proposed methods are very straightforward.}

\Ans{The challenges in leveraging tabular locality 
to query formula graphs lie in multiple aspects 
beyond just compressing formula graphs. 
We need to additionally develop algorithms for directly 
querying the compressed graphs without decompression 
and incrementally maintaining the compressed graphs. 
For example, in Sec.~\ref{sec:keyfunctions}, 
we have shown that developing the algorithms 
to efficiently query and maintain compressed edges 
for each basic pattern is non-trivial. 

In addition, while the heuristics for compressing formula graphs 
in Sec.~\ref{sec:sys} are indeed simple, they are derived from our 
observation from real-world spreadsheets and are effective in 
reducing graph sizes and the time for 
finding dependents and precedents, as shown in our experiments. 

In the revised paper, we have more clearly 
highlighted that there are challenges in compressing, querying, 
and maintaining formula graphs 
in the introduction (\fpointer{2}{1}{97}). 
}

\Rev{O3}{Comparing Excel with DataSpread is not very fair. First, Excel does not optimize for compressing formula graphs. Second, DataSpread is a light-weight system that is heavily customized for formula graphs. The experimental results are evident.}

\Ans{We agree that Excel is a complex system. 
It is possible that Excel has overhead that Dataspread does not have 
or that Excel is optimized for other scenarios 
by sacrificing the performance of finding dependents and precedents. 
For example, in our original paper, we identified 
one possible reason: Excel compresses formula graphs 
to reduce memory consumption but has to 
perform decompression in order to query the graphs. 
In the revised paper, we now acknowledge the possible overhead 
introduced by the complexity of Excel (\fpointer{12}{1}{1021}). 

However, we still see the value of this experiment since Excel 
is regarded as the state-of-the-art spreadsheet system and 
there is potential to improve Excel 
if the techniques of \sys are integrated. 
If the reviewer feels strongly that this comparison is unfair, 
we are happy to remove it from the paper.
}

\Rev{O4}{In conclusion, I agree that this is a practical problem, but only to those platforms with a huge number of users, such as Excel. If Excel wants to optimize this problem, any reasonable heuristic should be able to see clear impact. Hence, I want to see a justification that how this technique can be possibly grounded.}

\Ans{As mentioned in the response to \textbf{R3.O2}, 
we believe our contributions are beyond the heuristics 
for compressing formula graphs. We have developed 
novel algorithms for directly querying 
and incrementally maintaining compressed formula graphs, 
which can be used by Excel and other spreadsheet 
systems when they plan to leverage tabular locality to 
compress formula graphs.

Moreover, even without modifying Excel internals, 
our techniques can also be used to help Excel users. 
As mentioned in the response to \textbf{R3.O1}, 
one application for querying spreadsheet formula graphs is 
when users want to find and visualize the dependents and 
precedents of cells to check the accuracy of formulae and
identify sources of errors. 
Therefore, in the short term, we believe the techniques of 
\sys can be used by Excel users to support this application. 
We have implemented such a plug-in in Excel that is supported 
by \sys. The demo video is shown here:
\url{https://youtu.be/qxZWVJ7THjw}. 
In the long term, we expect the techniques of \sys 
to be integrated into modern spreadsheet systems, 
such as Google Sheets, LibreOffice Calc, and Microsoft Excel. 
In our prior efforts, we have discussed with the Google Sheets 
team about how to incorporate our findings and ideas into their system. 

In Sec.~\ref{sec:benchmark_config} of the revised paper, 
we now discuss how the techniques of \sys can be adopted to help 
spreadsheet users (\fpointer{9}{2}{809}).
}






==> sec-compact.tex <==
\section{Using Compact Representation in Computation Engine}
\label{sec:comp-compact}

The spreadsheet computation engine needs to be able to perform
the following two operations upon an update of a cell $c$:
\begin{enumerate}
    \item identify cells whose values are impacted by changing $c$, and
    \item recalculate the values of those impacted cells.
\end{enumerate}
Synchronous computation engines such as in Microsoft Excel may
perform these two operations together. However, other systems
such as \system may benefit from performing these two operations
separately on large spreadsheets, as described in the previous chapter.

\subsection{Dependency Graphs}
A dependency graph is used to represent the dependencies between
spreadsheet formula. We use the same definitions of dependencies
and dependency graphs as previously given in Section~\ref{sec:std_term}.

As discussed in the previous chapter, identifying cell dependencies
can be a lengthy process if done naively.
Certain dependency structures, such as long chains,
can be particularly tricky to manage.
Section~\ref{sec:graph-compression} introduces the
\emph{compressed dependency table} that helps mitigate issues of
long dependency identification time.
However, the compression heuristics might not perform well for
some sheet structures,
the size of the compressed dependency table can be
significantly larger than the actual complexity of the sheet, and
update propagation might take some time.

The formula graph, as defined above, can be extremely large.
A factor that contributes to its size is that a succinctly-written
range reference can spawn many edges; \code{B1=SUM(A1:A10000)} creates
$10\kilo$ edges, even if the formula string itself is relatively short.

\subsection{Compressed Dependency Data Structure}
The compressed dependency data structure internally represents
repeated edges in a more succinct fashion. First, we focus on
the pattern of repetition in the same column, where a
contiguous $n\times 1$ region (``starting region'') of cells
have one of the following patterns:
\begin{figure*}[ht]
    \centering
    \input{fig/ex-edge-types}
\caption{Compressed Edge Types}
\label{fig:edgetypeexample}
\end{figure*}
\begin{enumerate}
    \item \stitle{Moving-beginning Moving-ending (MM, ``sliding window'')}:
    edge $\mathrm{MM}(r, c, w)$ encodes the set of edges where
    the $i$-th cell of the starting region has a range reference to
    $(r_1+i, c):(r_2+i, c)$,
    \item \stitle{Stationary-beginning Moving-ending (SM, ``expanding window'')}:
    edge $\mathrm{SM}(r, c, w)$ encodes the set of edges where
    the $i$-th cell of the starting region has a range reference to
    $(r_1, c):(r_2+i, c)$,
    \item \stitle{Moving-beginning Stationary-ending (MS, ``shrinking window'')}:
    edge $\mathrm{MS}(r, c, w)$ encodes the set of edges where
    the $i$-th cell of the starting region has a range reference to
    $(r_1+i, c):(r_2, c)$,
    \item \stitle{Stationary-beginning Stationary-ending (SS, ``fixed window'')}:
    edge $\mathrm{SS}(r, c, w)$ encodes the set of edges where
    every cell of the starting region has a range reference to
    $(r_1, c):(r_2, c)$,
\end{enumerate}
where $r_1=r$ and $r_2=r+w-1$. Here, $(r, c)$ is the beginning cell,
and $w$ is the beginning window size of the
range referred to by the first cell in the starting region.

\begin{figure}[ht]
    \centering
    \input{fig/ex-chain}
\caption{Chain Edge}
\label{fig:chainexample}
\end{figure}
There is also a special case, \textbf{Chain (C)}, which
can be considered a special case of MM or SM,
where it is a sliding window of width $1$ that points to
cells within the starting region itself; that is,
when the $i$-th cell of the starting region has a reference to
the $(i-1)$-th cell of the starting region. When considering
dependencies, all the previous cells
along the chain must be included.


==> sec-dataset.tex <==
\section{Spreadsheet Complexity}
\label{sec:comp-dataset}

In large spreadsheets that contain many formulae, those formulae are
probably not all distinct.
It is extremely unlikely that large spreadsheets that have thousands
of formula come from users laboriously typing a formula in each cell
one-by-one, asking thousands of queries that are completely distinct
in nature.
Similar to typical software programming where loops and
iterations are ubiquitous,
these spreadsheets that contain numerous formula cells
more likely have similar computations being done multiple times,
possibly to different data points.
This is usually achieved by using the copy or auto-fill feature to
duplicate the formula to all the relevant cells.
Recognizing which cells perform the same computation can be useful
for improving the performance of the formula computation engine.

In this section, we analyze a dataset of real-world spreadsheets
in order to substantiate the claim that most spreadsheets with a large
number of formula actually contain only a handful of
essentially distinct formulae, just duplicated. We describe how
to utilize the findings to improve formula computation engines
in later sections.

\subsection{Essentially Identical Formulae}
\begin{figure}[h]
    \centering
    \input{fig/ex-copy}
\caption{Copy and auto-fill operations automatically
adjust relative references. (a) copying from cell
\code{A1} to cell \code{A4} (b) auto-filling from cell \code{A1}
down through cell \code{A4}}
\label{fig:copyexample}
\end{figure}
We define the notion of \emph{essentially identical formulae}
in order to help measure spreadsheet complexity.
The goal of such measure is to eliminate duplicate formulae
that are created using the copy or auto-fill operations
in spreadsheet applications.
When the user performs such operations,
formulae are duplicated to the target cell(s),
but the relative references are automatically adjusted so
that they keep the same relative distance, and the formula
string would appear different.
We use the ``standardized reference'' to discuss the essence of
what is kept identical when copied or auto-filled.

A (standardized) \emph{cell reference} $R=(r', c')$ of a cell $C=(r, c)$ has two components:
the row component $r'$, and the column component $c'$. Each component
can be \emph{relative} or \emph{absolute}, the latter denoted
with the prefix \texttt{\$}. A \emph{range reference}.
The cell reference $R$ \emph{resolves} to cell $R(C)=(r^*, c^*)$
where row $r^*$ is
\[r^*=
\begin{cases}
r'&\text{if $r'$ is an absolute reference}\\
r+r'&\text{if $r'$ is a relative reference}\\
\end{cases}\]
and column $c^*$ is defined similarly.
For example, let cell \code{A5} have the formula \code{=C\$1+7},
containing a reference to \code{C\$1}.
Here, it is a standardized reference $R=(\$1, +2)$
of cell $C_1=(5, 1)$, which resolves to cell $R(C_1)=(1, 3)$.
When this formula is copied over to cell {B6}, it will automatically
be adjusted to \code{=D\$1+7}. The standardized reference remains
$R=(\$1, +2)$, but from cell $C_2=(6, 2)$, it resolves to cell
$R(C_2)=(1, 4)$.

A (standardized) \emph{range reference} $R_1\code{:}R_2$
of a cell $C$, where $R_1$ and $R_2$
are cell references such that $R_1(C)=(r_1^*,c_1^*)$ and
$R_2(C)=(r_2^*,c_2^*)$,
resolves to all cells $(r^*,c^*)$ such that $r^*$ is between
$r_1^*$ and $r_2^*$, inclusive, and $c^*$ is between
$c_1^*$ and $c_2^*$, inclusive.

Two formulae from cells $C_1$ and $C_2$ are \emph{essentially identical} (EI)
if they are identical when the references are standardized according
to the corresponding cell. For example, of the following five cells,
only \code{A1} and \code{A2} have EI-formulae.
\begin{align*}
    \code{A1} &= \code{C1+SUM(\$D\$1:D6)}\\
    \code{A2} &= \code{C2+SUM(\$D\$1:D7)}\\
    \code{A3} &= \code{C3+SUM(\$D\$1:D7)}\\
    \code{A4} &= \code{C4+SUM(\$D\$1:\$D9)}\\
    \code{A5} &= \code{C5+SUM(\$D\$1:D10)+25}
\end{align*}
Note that while \code{A2} and \code{A3} do not have
EI-formulae, they would have had if $\code{D7}$ in both formulae
were replaced by $\code{D\$7}$ or $\code{\$D\$7}$.
These almost-EI patterns sometimes exist in spreadsheet, possibly
from procedural generations. They have potential for compression
like those that are EI, but are somewhat more difficult to detect.

\subsection{The Enron Dataset}
To verify our hypothesis that most spreadsheets are limited in
complexity, we first roughly measure the complexity of the spreadsheets
within our dataset by counting how many
\emph{essentially identical formulae} there are.

The Enron dataset\cite{klimt2004introducing} contains spreadsheets
that are used for communications within the Enron corporation.

In the Enron dataset, a vast majority of spreadsheets contain
few essentially distinct formulae, showing a potential for a
compact representation of these formulae.


==> sec-prototype-old.tex <==
\section{Implementation}
\label{sec:implementation}
Next, we discuss the prototype of implementing \sys, 
and \sys's applicability and overhead.

\stitle{Prototype}
\sys is implemented as a Java library, 
which can be used by third-party tools to analyze formula dependencies 
or integrated into spreadsheet systems to accelerate formula computation. 
\sys takes an xls or xlsx file as input, 
leverages the POI library~\cite{poi} to parse it, 
and builds a compressed formula graph 
for the parsed dependencies. 
The compressed formula graph is implemented using an adjacency list. 
We build a R-Tree~\cite{r-tree} 
on the vertices of the formula graph  
to quickly find vertices that overlap with a given range. 
\sys provides interfaces of finding \sdeps or \sprecs of a range, 
and adding or deleting a dependency. 

We also integrate \sys into \ds~\cite{demo1, datamodels, dataspread-demo2}, 
an open-source spreadsheet system. 
\ds has a web-based spreadsheet interface, 
uses a web server to process the front-end requests, 
and employs PostgreSQL as its back-end storage manager~\cite{hutchins1985direct}.
\ds uses ZK Spreadsheet~\cite{zk_spreadsheet} as its formula engine. 

\ds uses an asynchronous execution model to process an update. 
It returns control to users after it has identified all of the 
\sdeps of an update and marked them dirty. 
A formula graph is used to find the \sdeps of an update. 
\sys acts as a drop-in replacement for this formula graph. 
\sys builds the compressed formula graph and R-Tree 
when a spreadsheet is loaded. 
When formula cells are updated, \ds internally 
interprets the updates as a sequence of deletes and updates of dependencies, 
and modifies the compressed formula graph and R-Tree correspondingly. 
\ds also supports storing the compressed formula graph 
in the database backend as a relation, 
where each tuple stores a compressed edge 
and captures attributes, including the spreadsheet name, 
\sprec, \sdep, pattern type, and metadata. 
R-Tree indices are built on the \sprec and \sdep attributes.

\stitle{Applicability}
As discussed in Section~\ref{sec:background}, \sys can improve the
interactivity of spreadsheet systems that 
adopt either synchronous and asynchronous execution model.
Specifically, \sys can be integrated into other spreadsheet systems, 
such as LibreCalc or MS Excel, 
because these systems similarly trace dependencies across formulae and raw values
~\cite{calc-dep-graph, excel-dep-graph, zk_spreadsheet}.
For example, LibreCalc~\cite{calc-dep-graph} 
traces the \lprecs of a formula cell. 
When the \lprec of a formula cell is updated, 
the system will broadcast the new values to the formula cell. 
Therefore, the trace information is a formula graph 
and can be optimized by \sys. 
While we are not aware of Excel's internals since it is proprietary, 
online docs~\cite{excel-dep-graph, excel-trace} indicate that 
they similarly adopt a formula graph to trace dependencies 
and can thereby benefit from \sys. 

Beyond the integration with existing spreadsheet systems, 
\sys can be adopted by third-party tools that 
audit formula dependencies~\cite{excel-audit} 
and help users quickly identify the sources of errors.
%Furthermore, the patterns identified by \sys can 
%be leveraged to identify the outlier formulae and 
%automatically suggest potential errors, 
%which is the future work of \sys. 

\stitle{Overhead} 
As in general data compression, 
\sys introduces the overhead of formulae graph compression
and maintenance. 
However, compressing the formulae graph is performed 
when a spreadsheet is loaded into the system 
and is not on the critical path of users interacting 
with a spreadsheet. 
In addition, the time of maintaining a compressed formula graph is low 
as we will show in Section~\ref{sec:exp_build_graph} 
(e.g., less than 200 ms for deleting 1K formulae 
in the most complex graphs), 
and does not harm interactivity. 
Note that this overhead brings the benefit 
of significantly reducing the time of querying the graph. 
When we have large spreadsheets 
and the formula graphs are materialized to secondary storage, 
\sys has the benefit of using a smaller number of I/O operations to 
write/read the formula graph, 
which brings the overall compression and maintenance time 
lower than no compression as we will show in Section~\ref{sec:exp_build_graph}. 

\begin{comment}
Finally, if a spreadsheet shows less tabular locality, 
\sys has less performance benefit of querying the graph. 
However, Section~\ref{sec:exp_graph_size} 
shows that the tabular locality is prevalent in real-world spreadsheets 
and by leveraging this property 
\sys can significantly reduce the sizes of formula graphs 
and reduce the time of querying the graphs.
\end{comment}
